Continual Semantic Segmentation via Repulsion-Attraction of Sparse and Disentangled Latent Representations

Deep neural networks suffer from the major limitation of catastrophic forgetting old tasks when learning new ones. In this paper we focus on class incremental continual learning in semantic segmentation, where new categories are made available over time while previous training data is not retained. The proposed continual learning scheme shapes the latent space to reduce forgetting whilst improving the recognition of novel classes. Our framework is driven by three novel components which we also combine on top of existing techniques effortlessly. First, prototypes matching enforces latent space consistency on old classes, constraining the encoder to produce similar latent representation for previously seen classes in the subsequent steps. Second, features sparsification allows to make room in the latent space to accommodate novel classes. Finally, contrastive learning is employed to cluster features according to their semantics while tearing apart those of different classes. Extensive evaluation on the Pascal VOC2012 and ADE20K datasets demonstrates the effectiveness of our approach, significantly outperforming state-of-the-art methods.

==> sections/results_backup.tex <==
\section{Experimental Results}
\label{sec:results}

%\textbf{Continual Learning Baselines.} 
% alternatives: https://acronymify.com/search?q=Repulsion+Attraction+Sparse+Disentangled+Representations
We evaluate the performance of our method (denoted in the tables with \textbf{SDR}, i.e., Sparse and Disentangled Representations) against some state-of-the-art continual learning frameworks. We report as a lower limit the performance of the na\"ive fine-tuning approach (FT), which consists in training the model on the newly available training data with no additional provisions, while the upper limit is given by the offline single-shot training (offline) on the whole dataset $\mathcal{T}$ and on all the classes at once. Then, we compare with 3 recent continual semantic segmentation schemes: namely, ILT \cite{michieli2019incremental}, which combines latent and output level knowledge distillation, CIL \cite{klingner2020class}, which adds class importance weighting to output-level knowledge distillation, and MiB \cite{cermelli2020modeling}, which deals with the background distribution shift and proposes an unbiased weight initialization rule.
We also report the results of a few continual image classification algorithms adapted to semantic segmentation. Following \cite{cermelli2020modeling}, we consider some penalty computing approaches like Elastic Weight Consolidation (EWC) \cite{kirkpatrick2017overcoming}, %which uses the empirical Fisher matrix, 
Path Integral  (PI) \cite{zenke2017continual} %which uses the  learning trajectory, 
and Riemannian
Walks (RW) \cite{chaudhry2018riemannian} %, which combines the two ideas. 
and a couple of knowledge distillation approaches such as LwF \cite{li2018learning} %, which combines standard cross-entropy with output-level knowledge distillation, 
and its single-headed version LwF-MC \cite{rebuffi2017icarl}. For a fair comparison, all the methods have been re-trained with a standard Deeplab-v3+ \cite{deeplabv3plus2018} architecture with ResNet-101 \cite{he2016deep} as backbone.



\begin{table*}[t]
  \centering
  \caption{Quantitative results of mIoU over multiple incremental scenarios and experimental protocols on Pascal VOC2012. Best in \textbf{bold}, runner-up \underline{underlined}}
  \setlength{\tabcolsep}{1.18pt}
  \footnotesize
    \begin{tabular}{l|ccc|ccc|ccc||ccc|ccc|ccc||ccc|ccc|ccc}
     & \multicolumn{9}{c||}{19-1}                                             & \multicolumn{9}{c||}{15-5}                                             & \multicolumn{9}{c}{15-1} \\
          & \multicolumn{3}{c|}{sequential} & \multicolumn{3}{c|}{disjoint} & \multicolumn{3}{c||}{overlapped} & \multicolumn{3}{c|}{sequential} & \multicolumn{3}{c|}{disjoint} & \multicolumn{3}{c||}{overlapped} & \multicolumn{3}{c|}{sequential} & \multicolumn{3}{c|}{disjoint} & \multicolumn{3}{c}{overlapped} \\
          Method & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all   & old   & new   & all \\\hline
    FT    & 63.4  & 21.2  & 61.4  & 35.2  & 13.2  & 34.2  & 34.7  & 14.9  & 33.8  & 62.0  & 38.1  & 56.3  & 8.4   & 33.5  & 14.4  & 12.5  & 36.9  & 18.3  & 49.0  & 17.8  & 41.6  & 5.8   & 4.9   & 5.6   & 4.9   & 3.2   & 4.5 \\\hdashline
    PI \cite{zenke2017continual}   & 63.8  & 20.7  & 61.8  & 36.5  & 13.7  & 35.4  & 35.8  & 17.1  & 34.9  & 62.0  & 37.7  & 56.2  & 8.3   & 33.5  & 14.3  & 11.9  & 35.6  & 17.6  & 50.2  & 19.7  & 42.9  & 5.9   & 4.9   & 5.6   & 4.9   & 3.0   & 4.5 \\
    EWC \cite{kirkpatrick2017overcoming}  & 70.3  & \textbf{38.1}  & \underline{68.8}  & 55.8  & \underline{32.5}  & 54.7  & 57.2  & 29.0  & 55.9  & 67.4  & 44.7  & 62.0  & 8.4   & 32.8  & 14.2  & 32.8  & 42.5  & 35.1  & \underline{65.8}  & \textbf{31.9} & \underline{57.7}  & 15.6  & 14.3  & 15.3  & 9.3   & 4.2   & 8.1 \\
    RW \cite{chaudhry2018riemannian}   & \underline{70.5} & \underline{37.6}  & \textbf{69.0}  & 54.8  & 31.4  & 53.7  & 56.9  & \underline{31.2} & 55.7  & 67.6  & 44.2  & 62.0  & 8.4   & 33.4  & 14.3  & 31.3  & 39.5  & 33.3  & \textbf{66.6}  & \underline{31.7}  & \textbf{58.3}  & 17.5  & \textbf{17.5}  & 17.5  & 10.9  & \underline{16.1}  & 12.2 \\
    LwF  \cite{li2018learning} & 67.2  & 26.4  & 65.3  & 65.8  & 28.3  & 64.0  & 62.6  & 23.4  & 60.8  & 68.0  & 43.0  & 62.1  & 39.7  & 33.3  & 38.2  & 67.0  & 41.8  & 61.0  & 33.7  & 13.7  & 29.0  & 26.2  & 15.1  & 23.6  & 24.0  & 15.0  & 21.9 \\
    LwF-MC \cite{rebuffi2017icarl} & 49.2  & 0.9   & 46.9  & 38.5  & 1.0   & 36.7  & 37.1  & 2.3   & 35.4  & 70.6  & 19.5  & 58.4  & 41.5  & 25.4  & 37.6  & 59.8  & 22.6  & 51.0  & 12.1  & 1.9   & 9.7   & 6.9   & 2.1   & 5.7   & 6.9   & 2.3   & 5.8 \\\hdashline
    ILT \cite{michieli2019incremental}  & 64.3  & 22.7  & 62.3  & 66.9  & 23.4  & 64.8  & 50.2  & 29.2  & 49.2  & 71.3  & \textbf{47.8}  & 65.7  & 31.5  & 25.1  & 30.0  & 69.0  & 46.4  & 63.6  & 49.2  & 30.3  & 48.3  & 6.7   & 1.2   & 5.4   & 5.7   & 1.0   & 4.6 \\
    CIL \cite{klingner2020class}  & 64.1  & 22.8  & 62.1  & 62.6  & 18.1  & 60.5  & 35.1  & 13.8  & 34.0  & 63.8  & 39.8  & 58.1  & 42.6  & 35.0  & 40.8  & 14.9  & 37.3  & 20.2  & 52.4  & 22.3  & 45.2  & 33,3  & \underline{15.9}  & 29.1  & 6.3   & 4.5   & 5.9 \\
    MiB  \cite{cermelli2020modeling} & 68.2  & 31.9  & 66.5  & 67.0  & 26.0  & 65.1  & \underline{69.6}  & 23.8  & \underline{67.4}  & 73.0  & 44.4  & 66.1  & 47.5  & 34.1  & 44.3  & 73.1  & 44.5  & 66.3  & 35.7  & 11.0  & 29.8  & 39.0  & 15.0  & 33.3  & 44.5  & 11.7  & 36.7 \\\hline
    SDR (ours)  & 68.4  & 35.3  & 66.8  & \underline{69.9}  & \textbf{37.3}  & \underline{68.4}  & 69.1  & \textbf{32.6}  & \underline{67.4}  & \underline{73.6}  & \underline{46.7}  & \underline{67.2}  & \underline{73.5}  & \textbf{47.3}  & \underline{67.2}  & \underline{75.4}  & \textbf{52.6}  & \underline{69.9}  & 58.5  & 10.1  & 47.0  & \underline{59.2}  & 12.9  & \underline{48.1}  & \underline{44.7}  & \textbf{21.8}  & \underline{39.2} \\
    SDR + MiB & \textbf{70.6}  & 24.8  & 68.5  & \textbf{70.8}  & 31.4  & \textbf{68.9}  & \textbf{71.3}  & 23.4  & \textbf{69.0}  & \textbf{74.6}  & 43.8  & \textbf{67.3}  &\textbf{ 74.6}  & \underline{44.1}  & \textbf{67.3}  & \textbf{76.3}  & \underline{50.2}  & \textbf{70.1}  & 58.1  & 11.8  & 47.1  & \textbf{59.4 } & 14.3  & \textbf{48.7 } & \textbf{47.3}  & 14.7  & \textbf{39.5} \\\hline
    offline & 75.5  & 73.5  & 75.4  & 75.5  & 73.5  & 75.4  & 75.5  & 73.5  & 75.4  & 77.5  & 68.5  & 75.4  & 77.5  & 68.5  & 75.4  & 77.5  & 68.5  & 75.4  & 77.5  & 68.5  & 75.4  & 77.5  & 68.5  & 75.4  & 77.5  & 68.5  & 75.4 \\
    \end{tabular}%
  \label{tab:voc_quantitative}%
\end{table*}%
%
%
%
%
%
\newcommand{\imgsize}{18.6mm}
\begin{figure*}[htbp]
\setlength{\tabcolsep}{0.7pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.6}
\centering
\begin{tabular}{ccccccccccc}
  
   \rotatebox{90}{\hspace{+4ex}19-1} &  
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_label.png} & 
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_FT.png} & 
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_LWF.png} & 
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_ILT.png} &
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_CIL.png} &
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_MiB.png} &
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_ours.png} &
   \includegraphics[width=\imgsize]{img/19-1/2007_002119_offline.png} \\ 
   
      \rotatebox{90}{\hspace{+4ex}15-5} &  
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_label.png} & 
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_FT.png} & 
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_LWF.png} & 
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_ILT.png} &
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_CIL.png} &
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_MiB.png} &
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_ours.png} &
   \includegraphics[width=\imgsize]{img/15-5/2007_002597_offline.png} \\ 
   
   
         \rotatebox{90}{\hspace{+4ex}15-1} &  
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_label.png} & 
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_FT.png} & 
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_LWF.png} & 
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_ILT.png} &
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_CIL.png} &
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_MiB.png} &
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_ours.png} &
   \includegraphics[width=\imgsize]{img/15-5s/2007_002728_offline.png} \\ 
   
   
   \rotatebox{90}{\hspace{+3ex}100-50} &  
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_label.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_FT.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_LWF.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_ILT.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_CIL.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_MiB.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_ours.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-50/ADE_val_00001988_offline.png} \\ 
   
   \rotatebox{90}{\hspace{+3ex}100-10} &  
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_label.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_FT.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_LWF.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_ILT.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_CIL.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_MiB.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_ours.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/100-10/ADE_val_00000004_offline.png} \\ 
   
   \rotatebox{90}{\hspace{+4ex}50-50} &  
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_RGB.jpg} &
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_label.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_FT.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_LWF.png} & 
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_ILT.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_CIL.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_MiB.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_ours.png} &
   \includegraphics[width=\imgsize]{img/suppl/ade/50-50/ADE_val_00000051_offline.png} \\ 
   
  &  RGB  &  label  &  FT  &  LwF \cite{kirkpatrick2017overcoming}  &  ILT \cite{michieli2019incremental}  &  CIL \cite{klingner2020class} & MiB \cite{cermelli2020modeling} & SDR (ours) & offline \\
  
\end{tabular}
\caption{Qualitative results of competing approaches in different scenarios on disjoint VOC 2012 and ADE20K (\textit{best viewed in colors}).}
\label{fig:voc_qualitative}
\end{figure*}

\subsection{Pascal VOC2012}
Following previous works \cite{shmelkov2017incremental,michieli2019incremental,michieli2020knowledge,cermelli2020modeling}, we design three main experiments adding one class (19-1), five classes at once (15-5) and five classes sequentially (15-1) added in alphabetical order. We report comprehensive results (on the three experimental protocols defined in Section \ref{subsec:protocols}) in Table~\ref{tab:voc_quantitative} (results are reported for \textit{old}, \textit{new} and \textit{all} classes at the end of all the training phases). 

We can already appreciate forgetting of previous classes and difficulties in learning new ones, when adding as little as one class (the \textit{tv/monitor} class is added) in the scenario 19-1. FT always leads to the worst results in terms of \textit{old}, \textit{new} and \textit{all} classes. Methods derived from image classification improve the performance especially in the sequential scenario, where no background shift occurs. In this setting they achieve mIoUs sometimes comparable to the proposed method. Incremental methods designed for semantic segmentation  show more stability across the experimental protocols, in particular MiB, that is specifically targeted to solve the disjoint and the overlapped scenarios. Our method (SDR)  significantly outperforms the other segmentation methods in the disjoint and overlapped scenarios (with a gap of more than $3\%$ against the best competing approach in the disjoint setup), while also achieving competitive results in the sequential setup. Further adding on top of our method the distillation model from the MiB framework (which we regard as the current state of the art approach for class incremental semantic segmentation), the results increase on all the scenarios, showing how the proposed techniques are complimentary with respect to previous schemes.

When moving to the addition of 5 classes at once (i.e., \textit{potted plant}, \textit{sheep}, \textit{sofa}, \textit{train}, \textit{tv/monitor}) we immediately notice an overall increased drop of performance of all compared methods, especially in the disjoint and in the overlapped protocols, due to the increased domain shift occurring when adding more classes at once with very variable content. In this and in the following scenario, indeed, we are adding to the model classes belonging to different macroscopic groups, according to \cite{pascalvoc2012}, which are responsible for a variegate distribution: three indoor classes (\textit{potted plant}, \textit{sofa} and \textit{tv/monitor}), one animal class (\textit{sheep}) and one vehicle class (\textit{train}). Ad-hoc methods for segmentation typically outperform classification ones but are always surpassed by our method, which in particular outrun all competing methods by more than $20\%$ in the disjoint scenario.

In the final scenario we add the last 5 classes sequentially in 5 consecutive learning steps. This approach leads to the largest accuracy drop being the model exposed to a reiterated addition of single classes, which are also coming from different semantic contexts.
In the sequential protocol, classification-based approaches like EWC and RW can effectively outperform other approaches, while our framework shows competitive results being at the same level of the best segmentation-based approaches (ILT and CIL). In the disjoint and in the overlapped scenarios all the methods heavily suffer from the semantic shift undergone by the background class. The best classification approach (LwF) shows a negative gap from $10\%$ to $15\%$  with respect to the best segmentation method (MiB). Our approach (SDR) is able to significantly increase the final mIoU in both scenarios, thanks to the novel features-level constraints which help the model to maintain high accuracy on old classes while learning new ones. %Again, the most impressive results are in the disjoint scenario where it  outperforms all competitors of around $15\%$ but also in the overlapped one the gain is large.

Visual results for each of the considered scenarios in the disjoint protocol are shown in the first three rows of Fig.~\ref{fig:voc_qualitative}, where our method is compared against the best classification method (LwF) and all the segmentation ones showing consistently best segmentation maps.
For example, our method does not mislead the \textit{bus} windows with \textit{tv/monitor} instances in row 1 as several competitors (which are more biased toward predicting the novel class), and it is the only one able to distinguish the \textit{bus} in row 2 and the \textit{car} in row 3 from the similar-looking \textit{train} class. Here, the \textit{train} class is added in the incremental step causing catastrophic forgetting of similar classes in competing approaches.


\begin{table}[t]
  \caption{mIoU over multiple incremental scenarios on disjoint setup of ADE20K. Best in \textbf{bold}, runner-up \underline{underlined}}
  \setlength{\tabcolsep}{1.3pt}
  \small
  \centering
    \begin{tabular}{|l|ccc|ccc|ccc|}
    \hline
          & \multicolumn{3}{|c|}{100-50} & \multicolumn{3}{c|}{100-10} & \multicolumn{3}{c|}{50-50} \\
          Method & old   & new   & all   & old   & new   & all   & old   & new   & all \\\hline
    FT    & 0.0   & 22.5  & 7.5   & 0.0   & 2.5   & 0.8   & 13.9  & 12.0  & 12.6 \\\hdashline
    LwF \cite{li2018learning}   & 25.0  & 23.9  & 24.6  & 5.4   & 5.6   & 5.5   & 32.2  & 22.9  & 26.0 \\
    LwF-MC \cite{rebuffi2017icarl} & 8.6   & 0.0   & 5.8   & 0.0   & 0.9   & 0.3   & 2.8   & 0.5   & 1.2 \\\hdashline
    ILT \cite{michieli2019incremental}  & 27.2  & 21.7  & 25.4  & 0.0   & 0.2   & 0.8   & \underline{41.9}  & 21.1  & 28.0 \\
    CIL \cite{klingner2020class}   & 0.0   & 22.5  & 7.5   & 0.0   & 2.0   & 0.6   & 14.0  & 11.9  & 12.6 \\
    MiB \cite{cermelli2020modeling}  & \textbf{37.6} & 24.7  & \underline{33.3}  & \underline{21.0} & 5.3   & 15.8  & 39.1  & 22.6  & 28.1 \\\hline
    SDR (ours) & 37.4  & \underline{24.8}  & 33.2  & \textbf{28.9} & \underline{7.4}   & \underline{21.7}  & 40.9  & \underline{23.8}  & \underline{29.5} \\
    SDR+MiB & \underline{37.5}  & \textbf{25.5} & \textbf{33.5} & \textbf{28.9} & \textbf{11.7} & \textbf{23.2} & \textbf{42.9} & \textbf{25.4} & \textbf{31.3} \\\hline
    offline & 43.9  & 27.2  & 38.3  & 43.9  & 27.2  & 38.3  & 50.9  & 32.1  & 38.3 \\\hline
    \end{tabular}%
  \label{tab:ade_quantitative}%
\end{table}%


\subsection{ADE20K}
Following  \cite{cermelli2020modeling} we split the dataset into disjoint image sets with the only constraint that a minimum number of images (i.e., 50) have labeled pixels on $\mathcal{C}_k$. Classes are ordered according to \cite{zhou2017scene}. In this comparison we consider the best performing classification methods (LwF and LwF-MC) and all the segmentation approaches. The scenarios we consider are the addition of the last 50 classes at once (100-50), of the last 50 classes 10 at a time (100-10) and of the last 100 classes in 2 steps of 50 classes each (50-50). The results are summarized in Table~\ref{tab:ade_quantitative}, where we can appreciate that the proposed approach outperforms competitors in every scenario, in particular with a larger gain when multiple incremental steps are performed. When adding 50 classes at a time the best classification method (i.e., LwF) achieves modest results but it is outperformed by the best segmentation methods (i.e., ILT and MiB), which in turn are always consistently surpassed by our framework. In the scenario 100-10, instead, classification approaches and almost all segmentation approaches (except for MiB) are unable to provide useful outputs leading to very poor results, while our method was able to stand out from competitors. Visual results for each scenario are reported as last rows of Fig.~\ref{fig:voc_qualitative}, which confirm our considerations showing how our approach produces less noisy predictions and does not overestimate the background as some of the competitors.


\subsection{Ablation Study}

\begin{table}[t]
\caption{Ablation in the disjoint scenario of Pascal VOC2012 15-1 in terms of mIoU.}
\vspace{0.1cm}
\label{tab:ablation}
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{cccccc|ccc}
$\mathcal{L}_{ce}$ & $\mathcal{L}_{pm}$  & $\mathcal{L}_{sp}$ & $\mathcal{L}_{cl}$  & $\mathcal{L}'_{kd}$ &$\mathcal{L}_{kd}$ & old & new & all \\\hline
\checkmark & & & & & & 5.8 & 4.9 & 5.6 \\
\checkmark & & & & \checkmark & & 30.0 & 11.0 & 25.4 \\
\checkmark & \checkmark & & & & & 18.7 & 9.0 & 16.4 \\
\checkmark & \checkmark & \checkmark & & & & 40.4 & 12.9 & 33.9 \\
\checkmark & \checkmark & \checkmark & \checkmark & & & 41.0 & 13.2 & 34.4 \\\hline
\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & 50.0 & \textbf{15.9} & 41.9 \\
\checkmark & \checkmark & \checkmark & \checkmark &  & \checkmark & \textbf{59.2} & 12.9 & \textbf{48.1} \\
\end{tabular}
\end{table}

To evaluate the contributions of each component, we report an ablation analysis in Table~\ref{tab:ablation} on the Pascal dataset in the  challenging 15-1 scenario. As already noticed, FT leads to a great degradation of accuracy. Early continual learning approaches in semantic segmentation use a classical output-level knowledge distillation \cite{michieli2019incremental,michieli2020knowledge,klingner2020class} which  show discrete benefits boosting the mIoU by almost $20\%$. Each of the proposed techniques significantly contributes to the final mIoU providing non-overlapping and mutual benefits. Matching the prototypes, sparsifying the features vectors and constraining them via the contrastive objective regularize the latent space bringing large improvements on both old and new classes. Introducing standard output-level knowledge distillation on top increases the accuracy on old classes mainly, and its unbiased version prevents forgetting even more accounting for the background shift across the incremental learning steps.


\begin{table}[t]
\caption{mIoU on classical (non-incremental) semantic segmentation benchmarks.}
\vspace{0.1cm}
\label{tab:standard_segmentation}
\setlength{\tabcolsep}{6pt}
\centering
\begin{tabular}{ccc|cc}
$\mathcal{L}_{ce}$ & $\mathcal{L}_{sp}$ & $\mathcal{L}_{cl}$  & mIoU$_\mathrm{VOC2012}$ & mIoU$_\mathrm{ADE20K}$ \\\hline
\checkmark & & & 75.4  & 38.3 \\
\checkmark & \checkmark  & & 75.8 & 38.7 \\
\checkmark & & \checkmark  & 75.8 & 38.8 \\
\checkmark & \checkmark & \checkmark  & \textbf{76.3} & \textbf{39.3} \\
\end{tabular}
\end{table}

Finally, we show that two of the proposed approaches (namely, sparsity and contrastive learning) may be beneficial also for the more general case of standard (i.e., non incremental) semantic segmentation. Hence, we conduct some additional experiments on Pascal VOC2012 and ADE20K, reported in Table~\ref{tab:standard_segmentation}, showing the clear benefit of the two components in this situation. On both datasets the outcome is consistent, gaining $0.9\%$ and $1\%$ respectively starting from an architecture (i.e., Deeplab-v3+) which is already at the state-of-the-art.

